An Adaptive Gas Cost Mechanism for Ethereum to Defend Against Under-Priced DoS Attacks

The gas mechanism in Ethereum charges the execution of every operation to ensure that smart contracts running in EVM (Ethereum Virtual Machine) will be eventually terminated. Failing to properly set the gas costs of EVM operations allows attackers to launch DoS attacks on Ethereum. Although Ethereum recently adjusted the gas costs of EVM operations to defend against known DoS attacks, it remains unknown whether the new setting is proper and how to configure it to defend against unknown DoS attacks. In this paper, we make the first step to address this challenging issue by first proposing an emulation-based framework to automatically measure the resource consumptions of EVM operations. The results reveal that Ethereum's new setting is still not proper. Moreover, we obtain an insight that there may always exist exploitable under-priced operations if the cost is fixed. Hence, we propose a novel gas cost mechanism, which dynamically adjusts the costs of EVM operations according to the number of executions, to thwart DoS attacks. This method punishes the operations that are executed much more frequently than before and lead to high gas costs. To make our solution flexible and secure and avoid frequent update of Ethereum client, we design a special smart contract that collaborates with the updated EVM for dynamic parameter adjustment. Experimental results demonstrate that our method can effectively thwart both known and unknown DoS attacks with flexible parameter settings. Moreover, our method only introduces negligible additional gas consumption for benign users.

==> deploy.tex <==
\section{Discussion on Deployment}
\label{sec_deploy}
We suggest two ways to deploy our gas cost mechanism in practice (i.e., the public Ethereum blockchain), one mild and one more aggressive. Both approaches need the cooperation of a specific smart contract with Ethereum clients. For the mild approach, we need to write and deploy a smart contract that maintains the list of $\mu_i$ and takes actions (e.g., record, report) if DoS attacks are discovered. Note that the list is evolving with the increasing of normal transactions. On the client slide, a new module is required to download the list from the smart contract periodically, detect over-frequent operations, and send an alarm to the smart contract if such operations are found. Note that this approach does not change the gas costs. Instead, it detects DoS attacks based on our core idea (Section \ref{sec_method}).

The aggressive approach needs a smart contract to maintain the list of $\mu_i$ for the same reason. The client also downloads the list from the smart contract periodically and the way to modify the client is presented in Section \ref{sec_implementation}. The aggressive approach can prevent DoS attacks at the price of a hard fork due to the change of gas costs. In simple words, a hard fork splits the Ethereum blockchain into two, that may be troublesome since users can stay on the old chain if they are not willing to migrate to the new chain. %Moreover, hard fork is at risk of a new kind of replay attacks (i.e., if an account \emph{A} sends another account \emph{B} some Ether on the new chain, it is therefore possible to replay the same transaction on the old chain and vice versa)~\cite{replay_attack}.

